A mixed-integer programming model for identifying intuitive ambulance dispatching policies

Markov decision process models and algorithms can be used to identify optimal policies for dispatching ambulances to spatially distributed customers, where the optimal policies indicate the ambulance to dispatch to each customer type in each state. Since the optimal solutions are dependent on Markov state variables, they may not always correspond to a simple set of rules when implementing the policies in practice. Restricted policies that conform to a priority list for each type of customer may be desirable for use in practice, since such policies are transparent, explainable, and easy to implement. A priority list policy is an ordered list of ambulances that indicates the preferred order to dispatch the ambulances to a customer type subject to ambulance availability. This paper proposes a constrained Markov decision process model for identifying optimal priority list policies that is formulated as a mixed integer programming model, does not extend the Markov state space, and can be solved using standard algorithms. A series of computational examples illustrate the benefit of intuitive policies. The optimal mixed integer programming solutions to the computational examples have objective function values that are close to those of the unrestricted model and are superior to those of heuristics.

==> extensions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A MIP model with customer queues}\label{section:mipq}
The MIP model developed in Section \ref{section:mip} can be extended
to allow for customer queues to form, thus lifting one of the
simplifying assumptions.  The unrestricted MDP model
can be extended to include a customer queues; however, this would
expand the state space. As a result, policies may depend on who is
waiting in the queue, which may be undesirable if simple policies
are preferred. One of the benefits of using priority lists in the
presence of customer queues is that optimal policy does not depend
on who is in the queue. Model PL is extended here to allow for
customer queues, and the resulting model is labeled Model PLQ. It is
assumed that there is a known, deterministic approach for adding and removing
customers from a queue (e.g., a customer is served when a server
becomes available) such that the decision variables here only capture the
dispatching policies.

In Model PLQ, the states and decision variables are extended to
consider the possibility of a queue for customers that arrive when
all servers are busy. Let $Q$ denote the set of possible finite
queues that are allowed. The linear decision variables are
$y(s,w,j,q)$, which capture the proportion of time the system is in
state $s$ when customer $w$ has arrived and action $j$ is selected
with queue $q$. Likewise, the action sets, rewards, transition
probabilities are extended to add customers to the queue when all
servers are busy and to remove customers from the queue when
appropriate, yielding $X(s,w,q)$, $r(s,w,j,q)$, and $p(s', w',
q'|s,w,j,q)$, respectively. Adding a customer to the
queue is a null action here. The rewards for assigning servers to
servers to new customers is the same as in Model PL. To maintain realism, assume that
the reward accrued when assigning a server to a customer who has
been waiting in the queue is no more than the reward if the same
server immediately responds, such that there is not a net benefit for adding patients to the queue.
However, this assumption is not required to formulate or solve the model.
Note that Model PLQ is recurrent as
before. Define $P_{s,w,q}=m-|X(s,w,q)|+1$.  Model PLQ is formally
stated.
\begin{eqnarray}
% \nonumber to remove numbering (before each equation)
\mathrm{Model\ PLQ} &\max & \sum_{s \in S, w \in W, q \in Q, j \in
X(s,w,q)} \!\!\!\!\!\!\!\!\!\!\!\!r(s,w,j,q)\, y(s,w,j,q) \\
\nonumber \mathrm{subject\ to}&& \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\sum_{j' \in
X(s',w',q')} \!\!\!\!\!\! y(s',w',j',q') - \!\!\!\!\!\!\sum_{s \in S, w \in W, q
\in Q, j \in X(s,w,q)} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!p(s', w', q'|s,w,j,q)\,
y(s,w,j,q)= 0, \\
 && \hspace{2.0in} \mathrm{for}\ s' \in S, w' \in W, q' \in Q\\
 && \sum_{s \in S, w \in W, q \in Q, j \in X(s,w,q)}
\!\!\!\!\!\!\!\!\!\!\!\! y(s,w,j,q)=1
\end{eqnarray}
\begin{eqnarray}
  && y(s,w,j,q) \ge 0, s \in S, w \in W, q \in Q, j \in X(s,w,q) \\
  && \sum_{p=1}^m z_{w,j}^p = 1, w \in W^+, j=1,2,...,m\\
  && \sum_{j=1}^m z_{w,j}^p = 1, w \in W^+, p=1,2,...,m
%\label{mipmodel} && y(s,w,j) \le \sum_{p=1}^{P_{s,w}}\!\!\!\!\!\!\!\!\!\! z_{w,j}^p, s \in S,w \in W^+, j \in X^+(s,w)
\end{eqnarray}
\begin{eqnarray}
\nonumber && y(s,w,j,q) \le 1 - \!\!\!\!\!\!\!\!\!\!\sum_{j' \in X^+(s,w,q)}
\!\!\!\!\! z_{w,j'}^p + \sum_{p'=1}^{p-1} z_{w,j}^{p'},\ \mathrm{for}\ s \in S,q \in Q, \\
 && \hspace{1.0in} w \in W^+, j \in
X^+(s,w,q), p=1,2,...,P_{s,w,q} \\
 && z_{w,j}^p \in \{0,1\}, w \in W^+, j=1,2,...,m, p=1,2,...,m.
\end{eqnarray}

The objective function and constraints are analogous to those in Model PL.


%\subsection{A MIP model that allows idling}\label{section:mipidling}
%The non-idling policy assumption can be lifted for some types of
%customers to allow for the action space to allow for some customers
%to be ``lost.'' In the presence of queues, customers could either
%receive no service or be added to the queue when a server is
%available to delay service. We consider both of these scenarios
%here. For simplicity, we assume that an idling policy can be used
%for all customer types. However, allowing an idling policy for only
%some types of customers (such as low-priority customers) is
%straightforward. As for model PLQ, we assume that there is a known,
%deterministic policy in place for moving customers out of the queue.
%
%The additional actions of idling (server 0) or delaying service
%(server $m+1$), result in a total of $m+2$ servers. The objective is
%to add these two new actions to each customer type's priority list
%(of length $m+2$); however, these two new ``servers'' do not change
%the state space. The idling action is modeled as a server that is
%always available for certain types of customers. Therefore, the
%actions that appear in the priority list after the idling action are
%never selected. The action for delaying service (i.e., queuing) is
%not available in states that have a full queue (recall that we
%assume a finite queue). To maintain a recurrent MDP, we only allow
%idling for low-priority customers at each location.
%
%Define $P_{s,w,q}=(m+2)-|X(s,w,q)|+1$.
%
%Model PLIQ is formally stated. FIX TO ONLY ALLOW IDLING FOR
%LOW-PRIORITY CUSTOMERS.
%
%\begin{eqnarray}
%% \nonumber to remove numbering (before each equation)
%\nonumber \mathrm{Model\ PLIQ} &\max_x & \sum_{s \in S, w \in W, q \in Q, j \in X(s,w,q)} \!\!\!\!\!\!\!\!\!\!\!\!r(s,w,j,q)\, y(s,w,j,q) \\
%\nonumber \mathrm{subject\ to}&& \!\!\!\!\!\!\!\!\!\!\!\!\sum_{j' \in X(s',w',q')} \!\!\!\!\!\! y(s',w',j',q') - \!\!\!\!\!\!\sum_{s \in S, w \in W, q \in Q, j \in X(s,w,q)} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!p(s', w', q'|s,w,j,q)\, y(s,w,j,q)= 0, \\
%\nonumber && \hspace{3.0in} \mathrm{for}\ s' \in S, w' \in W, q' \in Q\\
%\nonumber && \sum_{s \in S, w \in W, q \in Q, j \in X(s,w,q)}\!\!\!\!\!\!\!\!\!\!\!\! y(s,w,j,q)=1\\
%\nonumber  && y(s,w,j,q) \ge 0, s \in S, w \in W, q \in Q, j \in X(s,w,q) \\
%\nonumber  && \sum_{p=1}^{m+1} z_{w,j}^p = 1, w \in W^+, j=0,1,...,m+1\\
%\nonumber  && \sum_{j=0}^{m+1} z_{w,j}^p = 1, w \in W^+, p=1,2,...,m+2\\
%%\label{mipmodel} && y(s,w,j) \le \sum_{p=1}^{P_{s,w}}\!\!\!\!\!\!\!\!\!\!z_{w,j}^p, s \in S,w \in W^+, j \in X^+(s,w)\\
%\nonumber && y(s,w,j,q) \le 1 - \!\!\!\!\!\!\!\!\!\!\sum_{j' \in X(s,w,q)\j}\!\!\!\!\! z_{w,j'}^p + \sum_{p'=1}^{p-1} z_{w,j}^{p'},\\
%\nonumber && \hspace{1.0in} \mathrm{for}\ s \in S,q \in Q, w \in W^+, j \in X^+(s,w,q), p=1,2,...,P_{s,w,q} \\
%\nonumber  && z_{w,j}^p \in \{0,1\}, w \in W^+, j=0,1,...,m+1, p=1,2,...,m+2.
%\end{eqnarray}
%
%The objective function and constraints are analogous to those
%in models PL and PLQ.


\subsection{A MIP model that allows idling}\label{section:mipidling}
In this section, we formulate Model PLIQ that lifts the non-idling policy assumption for the high-priority
customers to allow for the action space to allow for some customers
to be ``lost'' even when there are available servers. Here, we also allow for queues so that customers
could either receive no service due to idling or receive delayed
service due to queuing. Unlike in the previous section where
customers are added to the queue when all servers are busy, here
queuing is treated as a pseudo-server that allows customers to be
added to the queue at any time. To maintain a unichain MDP, we
assume that an idling policy can only be used only for the
low-priority customers. Note that the action for delaying service
(i.e., queuing) is not available in states that have a full queue
(recall that we assume a finite queue). Here, customers can be added
to a queue when there are servers available. Therefore, queuing in
Model PLIQ is distinct from queuing in Model PLQ.

As in model PLQ, we assume that there is a known, deterministic
policy in place for moving customers out of the queue. Therefore, we
partition the set of non-null customer types into low-priority (L)
and high-priority (H) subsets, i.e., $W^+ = W^+_L \cup W^+_H$, with
$W^+_L \cap W^+_H = \emptyset$. The additional idling action for
low-priority customers in $W^+_L$ are captured by server 0. The
additional action of delaying service through queuing is captured by
server $m+1$. Therefore, there are a total of $m+2$ ``servers'' that
are ordered for each type of customer, both of which are non-null
actions in states where there are available servers. These actions
are added to each low-priority customer type's priority list (of
length $m+2$); however, these two new ``servers'' do not change the
state space. The idling action is modeled as a server that is always
available for low-priority customers, and therefore, the actions that
appear in the priority list after the idling action (server 0) are
never selected. Idling is not allowed for high-priority customer
types, leading to at most $m+1$ actions (including queuing). Based
on these assumptions, define $P^L_{s,w,q}=(m+2)-|X(s,w,q)|+1$ and
$P^H_{s,w,q}=(m+1)-|X(s,w,q)|+1$. Model PLIQ is formally stated as (\ref{pliq1}) -- (\ref{pliq2}).
\begin{eqnarray}
% \nonumber to remove numbering (before each equation)
\label{pliq1}\mathrm{Model\ PLIQ} &\max & \sum_{s \in S, w \in W, q \in Q, j
\in
X(s,w,q)} \!\!\!\!\!\!\!\!\!\!\!\!r(s,w,j,q)\, y(s,w,j,q) \\
\nonumber \mathrm{subject\ to}&& \!\!\!\!\!\!\!\!\!\!\!\!\sum_{j' \in
X(s',w',q')} \!\!\!\!\!\! y(s',w',j',q') - \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\sum_{s \in S, w \in W, q
\in Q, j \in X(s,w,q)} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!p(s', w', q'|s,w,j,q)\,
y(s,w,j,q)= 0, \\
&& \hspace{2.0in} \mathrm{for}\ s' \in S, w' \in W, q' \in Q\\
 && \sum_{s \in S, w \in W, q \in Q, j \in X(s,w,q)}
\!\!\!\!\!\!\!\!\!\!\!\! y(s,w,j,q)=1\\
 && y(s,w,j,q) \ge 0, s \in S, w \in W, q \in Q, j \in X(s,w,q).
\end{eqnarray}
The next five sets of constraints set the priority list variables
for the low-priority customers that allow for idling and queuing.
\begin{eqnarray}
 && \sum_{p=1}^{m+1} z_{w,j}^p = 1, w \in W_L^+, j=0,1,...,m+1\\
 && \sum_{j=0}^{m+1} z_{w,j}^p = 1, w \in W_L^+, p=1,2,...,m+2\\
%\label{mipmodel} && y(s,w,j) \le \sum_{p=1}^{P_{s,w}}\!\!\!\!\!\!\!\!\!\! z_{w,j}^p, s \in S,w \in W^+, j \in X^+(s,w)\\
\nonumber && y(s,w,j,q) \le 1 - \!\!\!\!\!\!\!\!\!\!\sum_{j' \in X^+(s,w,q)}
\!\!\!\!\! z_{w,j'}^p + \sum_{p'=1}^{p-1} z_{w,j}^{p'},\\
 && \hspace{1.0in} \mathrm{for}\ s \in S,q \in Q, w \in W_L^+, j \in
X^+(s,w,q), p=1,2,...,P^L_{s,w,q} \\
  && z_{w,j}^p \in \{0,1\}, w \in W_L^+, j=0,1,...,m+1, p=1,2,...,m+2.
\end{eqnarray}
The final five sets of constraints set the priority list
variables for the high-priority customers that allow queuing
but not idling.
\begin{eqnarray}
 && \sum_{p=1}^{m+1} z_{w,j}^p = 1, w \in W_H^+, j=1,...,m+1\\
 && \sum_{j=0}^{m+1} z_{w,j}^p = 1, w \in W_H^+, p=1,2,...,m+1\\
%\label{mipmodel} && y(s,w,j) \le \sum_{p=1}^{P_{s,w}}\!\!\!\!\!\!\!\!\!\! z_{w,j}^p, s \in S,w \in W^+, j \in X^+(s,w)\\
\nonumber && y(s,w,j,q) \le 1 - \!\!\!\!\!\!\!\!\!\!\sum_{j' \in X^+(s,w,q)}
\!\!\!\!\! z_{w,j'}^p + \sum_{p'=1}^{p-1} z_{w,j}^{p'},\\
 && \hspace{1.0in} \mathrm{for}\ s \in S,q \in Q, w \in W_H^+, j \in
X^+(s,w,q), p=1,2,...,P^H_{s,w,q} \\
\label{pliq2} && z_{w,j}^p \in \{0,1\}, w \in W_H^+, j=1,...,m+1, p=1,2,...,m+1.
\end{eqnarray}
The objective function and constraints are analogous to those
in models PL and PLQ.

It is worth noting that in many server-to-customer systems, such as
emergency medical services, idling policies are not typically used,
since as all customers are expected to be served immediately or else
queued. However, low-priority patients are sometimes idled during
natural disasters or mass casualty events when the number of patients who
require service overwhelm the system.


